Regular Abstractions for Array Systems

Verifying safety and liveness over array systems is a highly challenging problem. Array systems naturally capture parameterized systems such as distributed protocols with an unbounded number of processes. Such distributed protocols often exploit process IDs during their computation, resulting in array systems whose element values range over an infinite domain. In this paper, we develop a novel framework for proving safety and liveness over array systems. The crux of the framework is to overapproximate an array system as a string rewriting system (i.e. over a finite alphabet) by means of a new predicate abstraction that exploits the so-called indexed predicates. This allows us to tap into powerful verification methods for string rewriting systems that have been heavily developed in the last few decades (e.g. regular model checking). We demonstrate how our method yields simple, automatically verifiable proofs of safety and liveness properties for challenging examples, including Dijkstra's self-stabilizing protocol and the Chang-Roberts leader election protocol.

==> correctness.tex <==
\section{Proof of Theorem \ref{thm:regular-abstraction-properties}}
\label{sec:main-theorem-proof}
Fix a set of indexed predicates $\pred{P} := \iset{ P_1, \ldots, P_m }$.
When $\phi$ is not singly indexed, we simply output a trivial regular abstraction like $(\Nat^r \times \Sigma_m^*, \pred{P})$.
Now suppose that $\phi := \partial x_1 \cdots \partial x_n.\,\varphi$ is a normalized SIA formula.
Our method first computes an intermediate formula $\psi := \partial x_1 \cdots \partial x_n.\,\Tilde{\varphi}$ by replacing the matrix $\varphi$ of $\phi$ with a quantifier-free formula $\Tilde{\varphi}$
such that $\varphi \Rightarrow \Tilde{\varphi}$ holds in $\theory$.
It is easy to see that $\alpha(\sem{\phi}_\structA) \subseteq \alpha(\sem{\psi}_\structA)$ for any model $\structA$ of $\theory$.
Moreover, $\psi$ is by construction expressible in the predicate language of $\pred{P}$, namely, each value expression in $\psi$ is an instantiation of a predicate (or its negation) in $\pred{P}$.
Our method then computes the abstraction formula as $\phi^\star = f(\psi)$, where $f(\cdot)$ denotes the transformation by replacing value expressions in the given formula with appropriate instantiations of the $\Delta_k$'s.
Now it is sufficient to show that for every model $\structA$ of $\theory$ and tuple $(t,w) \in \alpha(\sem{\psi}_\structA)$,
it holds that $(t,w) \in \sem{\phi^\star}_{\struct_m}$.

Consider a tuple $(t,w) \in \alpha(\sem{\psi}_\structA)$,
and define
$\Psi_{t,w} := \Phi_w^{\pred{P}} \wedge \bigwedge_{i=1}^r x_i = t_i$.
Since $(t,w) \in \alpha(\sem{\psi}_\structA)$,
we see that $\Psi_{t,w} \Rightarrow \psi$ holds in $\theory$.
This in turn implies that $f(\Psi_{t,w} \Rightarrow \psi)$ holds in $\struct_m$, as $\Psi_{t,w} \Rightarrow \psi$ is in the predicate language of $\pred{P}$.
However, notice that $f(\Psi_{t,w} \Rightarrow \psi)$
iff $f(\Psi_{t,w}) \Rightarrow f(\psi)$
iff $f(\Psi_{t,w}) \Rightarrow \phi^\star$.
Since $\struct_m, (t,w) \models f(\Psi_{t,w})$,
we have $\struct_m, (t,w) \models \phi^\star$, which
allows us to conclude that $(t,w) \in \sem{\phi^\star}_{\struct_m}$.


==> fairness.tex <==
\section{Liveness verification under fairness requirements}
We briefly discuss how to perform liveness verification
of an index-bounded array system
in the presence of fairness requirements, which are essential in specifying reactive and concurrent process systems (cf.~\cite{demri2016temporal,manna2012temporal}).

An~\emph{(abstractable) fairness specification}
is a temporal array property $\eta$
containing a designated index variable $i$
and constrained by the grammar
\begin{align*}
    \eta & ::= \GF \mu \mid \FG \mu \mid \eta \vee \eta \mid \eta \wedge \eta,
\end{align*}
where $\mu$ is an abstractable indexed array formula.
Let $\structT$ be an index-bounded array system defined over $\voc$,
and $\eta$ be a fairness specification.
Given a model $\structA$ of $T_A$,
a path $\pi := s_0\,s_1 \cdots$ is \emph{fair}
if $\structA, \pi \models \eta[t/i]$ for $1 \le t \le s_0(p)$
for a designated parameter $p \in \voc_{par}$.
A temporal array property $\phi$ holds for $\structT$
under a fairness specification if
$\structT$ does not have a fair path violating $\phi$.
We note that this formalism is expressive enough to capture typical fairness
requirements for concurrent systems, including
\emph{process fairness} (in form of $\GF \phi$),
\emph{weak fairness} (in form of $\GF \phi \vee \GF \psi$),
and \emph{strong fairness} (in form of $\GF \phi \vee \FG \psi$).
See e.g.~\cite{manna2012temporal} for a detailed discussion of these fairness requirements.

Given a fairness specification $\eta$ and indexed predicates $\pred{P}$,
we can compute a regular abstraction $(E,\pred{P})$
overapproximating $\eta$ in the abstract domain.
Namely, if there is a fair concrete path $s_0\, s_1 \cdots$ with respect to $\eta$,
then there is a fair abstract path $t_0\, t_1 \cdots$ with respect to $E$,
and $t_i \in \alpha(s_i)$ for each $i \ge 0$.
This abstract fairness condition $E$,
together with an abstract regular liveness property $(I,T,F)$,
can be automatically translated to a formalism similar to
the so-called \emph{B\"uchi regular transition system (BRTS)}~\cite{abdulla2012regular},
which generalizes the translation from linear temporal properties to
B\"uchi automata in finite-state model checking~\cite{vardi1986automata}.
Verifying the existence of fair counterexample paths then amounts to
searching for reachable loops that contain an accepting state,
which can in turn be reduced to a safety verification problem~\cite{schuppan2006liveness,daniel2016infinite}.
We provide technical details of the
translation and reduction procedures in Appendix~\ref{sec:safety-reduction}.
Together with Theorem~\ref{thm:regulation-abstraction-for-liveness},
we can summarize our results in this section as follows.
\begin{theorem}
 \label{thm:regulation-abstraction-for-liveness-2}
  Let $\structT$ be an index-bounded array system, $\phi$ be a liveness array property,
  and $\psi$ be a fairness specification.
  Suppose that $\structT$ and $\neg \phi$ are abstractable,
  and that $\structT$ is $\neg \phi$-progressing.
  Then we can compute finite automata $\cI$, $\cT$, and $\cF$,
  as well as a regular fairness requirement $\Psi$,
  such that $\phi$ holds for $\structT$ under the fairness specification $\psi$ if the liveness property $(\cI, \cT, \cF)$ holds under the fairness requirement $\Psi$.
\end{theorem}

==> semantics.tex <==
\section{Semantics of temporal array formulae}
\label{sec:semantics}
We provide below the semantics of temporal array formulae. Here $\pi := s_0\, s_1 \cdots$ is a path, and $\pi^t := s_{t}\,s_{t+1} \cdots$ denotes the suffix of $\pi$ starting at position~$t \ge 0$.
\begin{eqnarray*}
    \pi \models \phi & \mbox{ iff } &  s_0 \models \phi,\ \mbox{given that $\phi$ is an indexed array formula}\\
    \pi \models \neg\phi & \mbox{ iff } &  \pi \not\models \phi\\
    \pi \models \phi_1 \vee \phi_2 & \mbox{ iff } &
    \pi \models \phi_1\ \mbox{or}\ \pi \models \phi_2\\
    \pi \models \phi_1 \wedge \phi_2 & \mbox{ iff } &
    \pi \models \phi_1\ \mbox{and}\ \pi \models \phi_2\\
    \pi \models \exists i.\:\phi & \mbox{ iff } &
    \mbox{$i$ is an index variable and $\pi \models \phi [n/i]$ for some $n \in \Nat$}\\
    \pi \models \forall i.\:\phi & \mbox{ iff } &
    \mbox{$i$ is an index variable and $\pi \models \phi [n/i]$ for all $n \in \Nat$}\\
    \pi \models \G \phi & \mbox{ iff } & \mbox{for all $t \ge 0$, it holds that}\ \pi^t  \models \phi\\
    \pi \models \F \phi & \mbox{ iff } & \mbox{for some $t \ge 0$, it holds that}\ \pi^t  \models \phi
\end{eqnarray*}
